On Exact Sizes of Minimal CNOT Circuits

Computing a minimum-size circuit that implements a certain function is a standard optimization task. We consider circuits of CNOT gates, which are fundamental binary gates in reversible and quantum computing. Algebraically, CNOT circuits on $n$ qubits correspond to $GL(n,2)$, the general linear group over the field of two elements, and circuit minimization reduces to computing distances in the Cayley graph $G_n$ of $GL(n,2)$ generated by transvections. However, the super-exponential size of $GL(n,2)$ has made its exploration computationally challenging. In this paper, we develop a new approach for computing distances in $G_n$, allowing us to synthesize minimum circuits that were previously beyond reach (e.g., we can synthesize optimally all circuits over $n=7$ qubits). Towards this, we establish two theoretical results that may be of independent interest. First, we give a complete characterization of all isometries in $G_n$ in terms of (i) permuting qubits and (ii) swapping the arguments of all CNOT gates. Second, for any fixed $d$, we establish polynomials in $n$ of degree $2d$ that characterize the size of spheres in $G_n$ at distance $d$, as long as $n\geq 2d$. With these tools, we revisit an open question of [Bataille, 2022] regarding the smallest number $n_0$ for which the diameter of $G_{n_0}$ exceeds $3(n_0-1)$. It was previously shown that $6\leq n_0 \leq 30$, a gap that we tighten considerably to $8\leq n_0 \leq 20$. We also confirm a conjecture that long cycle permutations lie at distance $3(n-1)$, for all $n\leq 8$, extending the previous bound of $n\leq 5$.

==> lemma_alt.tex <==
    \begin{lemma} \label{Size of an orbit is a polynomial}
        Let $M\in X_m$, with $|\varepsilon(M)|=e$. Then 
        $$|\SymmetricGroup_n\cdot \phi_{mn}(M)|=|\SymmetricGroup_m\cdot M|\cdot \binom{m}{e}^{-1} \binom{n}{e}.$$
    \end{lemma}
    \begin{proof}
    We note firstly that we can reduce the lemma to the case where $|M|=m$. To see this assume $|\Essential(M)|=e$. By (todo:ref) we can find $M'\in X_e$ s.t. $\Embedding_{em}(M')$ lies in the same orbit as $M$. If we assume the lemma for $M'$ we then get
    \begin{align*}|S_n\cdot \Embedding_{m,n}(M)|&=|\SymmetricGroup_n\cdot \Embedding_{e,n}(M')|\\ &=|\SymmetricGroup_e\cdot M'|\cdot\binom{n}{e}\\
    &=|\SymmetricGroup_m\cdot \Embedding_{e,m}(M')|\cdot \binom{m}{e}^{-1}\binom{n}{e}\\
    &=|\SymmetricGroup_m\cdot M|\cdot \binom{m}{e}^{-1}\binom{n}{e}.
    \end{align*}
    Suppose therefore $\Essential(M)=[m]$. We must establish that
    $$|\SymmetricGroup_n\cdot \Embedding_{m,n}(M)|=|\SymmetricGroup_m\cdot M|\cdot \binom{n}{m}.$$
By the orbit-stabilizer theorem (\cref{eq:orbit_stabilizer_size}), we have that 
\[
\SymmetricGroup_n\cdot \Embedding_{m,n}(M)= \frac{|\SymmetricGroup_n|}{\Stabilizer(\Embedding_{m,n}(M))} = \frac{n!}{\Stabilizer(\Embedding_{m,n}(M))}
\]
We will now identify the stabilizer subgroup of $\Embedding_{m,n}(M)$, i.e., the set of permutations $\sigma\in\SymmetricGroup_n$ such that $\sigma\cdot \Embedding_{m,n}(M)=\Embedding_{m,n}(M)$.
Recall that  that $\Essential(M)=\Essential(\Embedding_{m,n})(M)$ (\cref{item:essential_invariant1} of \cref{lem:essential_indices_invariant}).
We distinguish the following two cases.

\SubParagraph{Case 1.}
Assume that $\sigma$ satisfies $\sigma(i)\in [m]$ iff $i\in [m]$, i.e., it only shuffles the essential indices of $\Embedding_{m,n}(M)$.
By \cref{item:essential_indeces_are_sufficient} of \cref{lem:essential_indices_are_essential}, there exists a circuit  $C=\prod_{k=1}^dT_{i_k,j_k}$ that evaluates to $\Embedding_{m,n}(M)$ and uses only the essential indices of $\Embedding_{m,n}(M)$.
By the definition of the group action, we have
\[
\sigma\cdot \left( \prod_{k=1}^dT_{i_k,j_k} \right) =  \prod_{k=1}^dT_{\sigma(i_k),\sigma(j_k)}
\numberthis\label{eq:size_of_orbit_is_polynomial_circuit}
\]
By our assumption on $\sigma$, the circuit on the right-hand side of \cref{eq:size_of_orbit_is_polynomial_circuit} only contains the essential indices of $\Embedding_{m,n}(M)$.
Hence, we can take the preimage of $\Embedding_{m,n}$ to obtain a circuit evaluating to some element in $\GL(m,2)$.
It is therefore not hard to see that $\sigma$ is a stabilizer of $\Embedding_{m,n}(M)$ if and only if $\sigma'$ is a stabilizer of $M$,
where $\sigma'$ is obtained by ignoring the indices $m+1, \dots, n$ in $\sigma$.

\SubParagraph{Case 2.}
Assume that there is at least one essential index $i\in [m]$ such that $\sigma(i)\not \in [m]$, i.e., $\sigma$ maps an essential index of $\Embedding_{m,n}(M)$ to a non essential index of $\Embedding_{m,n}(M)$.
Then $\sigma$ cannot be a stabilizer of $\Embedding_{m,n}(M)$, since we can again consider \cref{eq:size_of_orbit_is_polynomial_circuit}, and observe that at least one essential index of $M$ would be missing, meaning that $C$ cannot evaluate to $M$, due to \cref{item:essential_indeces_are_necessary} of \cref{lem:essential_indices_are_essential}.

Since the two cases are exhaustive, we conclude that  $\Stabilizer(\Embedding_{m,n}(M))$ are isomorphic to $\Stabilizer(M)\times \SymmetricGroup_{n-m}$ (i.e., only case 1 applies), to arrive at
\[
|\SymmetricGroup_n\cdot \Embedding_{m,n}(M)| = \frac{n!}{\Stabilizer(M)\times \SymmetricGroup_{n-m}} = \frac{n!}{\Stabilizer(M) \cdot (n-m)!} = |\SymmetricGroup_m\cdot M|\frac{n!}{m!\cdot (n-m)!}
\]
where the last step is obtained by applying the orbit-stabilizer theorem (\cref{eq:orbit_stabilizer_size}) stating that $m!=|\SymmetricGroup_m| = |\SymmetricGroup_M\cdot M| \cdot |\Stabilizer(M)|$.
\end{proof}
